A Hybrid Approach combining ANN-based and Conventional Demapping in Communication for Efficient FPGA-Implementation

In communication systems, Autoencoder (AE) refers to the concept of replacing parts of the transmitter and receiver by artificial neural networks (ANNs) to train the system end-to-end over a channel model. This approach aims to improve communication performance, especially for varying channel conditions, with the cost of high computational complexity for training and inference. Field-programmable gate arrays (FPGAs) have been shown to be a suitable platform for energy-efficient ANN implementation. However, the high number of operations and the large model size of ANNs limit the performance on resource-constrained devices, which is critical for low latency and high-throughput communication systems. To tackle his challenge, we propose a novel approach for efficient ANN-based remapping on FPGAs, which combines the adaptability of the AE with the efficiency of conventional demapping algorithms. After adaption to channel conditions, the channel characteristics, implicitly learned by the ANN, are extracted to enable the use of optimized conventional demapping algorithms for inference. We validate the hardware efficiency of our approach by providing FPGA implementation results and by comparing the communication performance to that of conventional systems. Our work opens a door for the practical application of ANN-based communication algorithms on FPGAs.

==> sections/03_case_study.tex <==
\section{Case Study}

\todo{Include implementation of previous paper as simple case-study: NN-structure, 16-QAM, SISO, low-latency, low-power, phase-offset channel...}


==> sections/06_future_work.tex <==
\section{Future Work}

\todo{Make clear that is was just a case-study with preliminary  results to present the methodology, not a complete system. In Future work will be applied to more realistic 5G system: MIMO, 256-QAM, real channel...}
